Observational constraints on dark energy cosmological model parameters

The expansion rate of the Universe changes with time, initially slowing (decelerating) when the universe was matter dominated, because of the mutual gravitational attraction of all the matter in it, and more recently speeding up (accelerating). A number of cosmological observations now strongly support the idea that the Universe is spatially flat (provided the dark energy density is at least approximately time independent) and is currently undergoing an accelerated cosmological expansion. A majority of cosmologists consider "dark energy" to be the cause of this observed accelerated cosmological expansion. The "standard" model of cosmology is the spatially-flat {\Lambda}CDM model. Although most predictions of the {\Lambda}CDM model are reasonably consistent with measurements, the {\Lambda}CDM model has some curious features. To overcome these difficulties, different Dark Energy models have been proposed. Two of these models, the XCDM parametrization and the slow rolling scalar field model $\phi$CDM, along with "standard" {\Lambda}CDM, with the generalization of XCDM and $\phi$CDM in non-flat spatial geometries are considered here and observational data are used to constrain their parameter sets. In this thesis, we start with a overview of the general theory of relativity, Friedmann's equations, and distance measures in cosmology. In the following chapters we explain how we can constrain the three above mentioned cosmological models using three data sets: measurements of the Hubble parameter $H(z)$, Supernova apparent magnitudes, and the BAO peak length scale, as functions of redshift $z$. We then discuss constraints on the deceleration-acceleration transition redshift $z_{\rm da}$ using unbinned and binned $H(z)$ data. Finally, we incorporate the spatial curvature in the XCDM and $\phi$CDM model and determine observational constraints on the parameters of these expanded models.

==> preface.tex <==
% +--------------------------------------------------------------------+
% | Preface (Optional)
% +--------------------------------------------------------------------+

\newpage
\begin{center}
{\bf \Huge Preface}
\end{center}
\vspace{1cm}
\setlength{\baselineskip}{0.8cm}

%\pdfbookmark[0]{Preface}{PDF_Preface}

% +--------------------------------------------------------------------+
% | Enter text of your Preface in the space below this box.
% +--------------------------------------------------------------------+

This template uses a separate file for each section of your ETDR:
title page, abstract, preface, chapters, reference, etc.  This
makes it easier to organize and work with a lengthy document.  The
template is configured with page margins required by the Graduate
School and will automatically create a table of contents, lists of
tables and figures, and PDF bookmarks.

Although the template gives you a foundation for creating your
ETDR, you will need a working knowledge of LaTeX in order to
produce a final document.  You should be familiar with LaTeX
commands for formatting text, equations, tables, and other
elements you will need to include in your ETDR.

This template uses a separate file for each section of your ETDR:
title page, abstract, preface, chapters, reference, etc.  This
makes it easier to organize and work with a lengthy document.  The
template is configured with page margins required by the Graduate
School and will automatically create a table of contents, lists of
tables and figures, and PDF bookmarks.

Although the template gives you a foundation for creating your
ETDR, you will need a working knowledge of LaTeX in order to
produce a final document.  You should be familiar with LaTeX
commands for formatting text, equations, tables, and other
elements you will need to include in your ETDR.

This template uses a separate file for each section of your ETDR:
title page, abstract, preface, chapters, reference, etc.  This
makes it easier to organize and work with a lengthy document.  The
template is configured with page margins required by the Graduate
School and will automatically create a table of contents, lists of
tables and figures, and PDF bookmarks.

Although the template gives you a foundation for creating your
ETDR, you will need a working knowledge of LaTeX in order to
produce a final document.  You should be familiar with LaTeX
commands for formatting text, equations, tables, and other
elements you will need to include in your ETDR.

